Inter-Frame Compression for Dynamic Point Cloud Geometry Coding

Efficient point cloud compression is essential for applications like virtual and mixed reality, autonomous driving, and cultural heritage. This paper proposes a deep learning-based inter-frame encoding scheme for dynamic point cloud geometry compression. We propose a lossy geometry compression scheme that predicts the latent representation of the current frame using the previous frame by employing a novel feature space inter-prediction network. The proposed network utilizes sparse convolutions with hierarchical multiscale 3D feature learning to encode the current frame using the previous frame. The proposed method introduces a novel predictor network for motion compensation in the feature domain to map the latent representation of the previous frame to the coordinates of the current frame to predict the current frame's feature embedding. The framework transmits the residual of the predicted features and the actual features by compressing them using a learned probabilistic factorized entropy model. At the receiver, the decoder hierarchically reconstructs the current frame by progressively rescaling the feature embedding. The proposed framework is compared to the state-of-the-art Video-based Point Cloud Compression (V-PCC) and Geometry-based Point Cloud Compression (G-PCC) schemes standardized by the Moving Picture Experts Group (MPEG). The proposed method achieves more than 88% BD-Rate (Bjontegaard Delta Rate) reduction against G-PCCv20 Octree, more than 56% BD-Rate savings against G-PCCv20 Trisoup, more than 62% BD-Rate reduction against V-PCC intra-frame encoding mode, and more than 52% BD-Rate savings against V-PCC P-frame-based inter-frame encoding mode using HEVC. These significant performance gains are cross-checked and verified in the MPEG working group.

==> authors_bio_portrait/Anique_Akhtar_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../authors_bio_portrait/Anique_Akhtar_portrait}}]{Anique Akhtar} is a senior engineer at Qualcomm Technologies Inc. in San Diego, CA, USA, in the Multimedia R\&D \& Standards group where he actively participates and contributes to the standardization efforts on MPEG's Point Cloud Compression (PCC) and Video-Based Dynamic Mesh Coding (V-DMC). Anique received his B.S. degree in Electrical Engineering from Lahore University of Management Sciences (LUMS), Lahore, Pakistan, in 2013, received his M.S. degree from Koc University, Istanbul, Turkey, in 2015, and received his Ph.D. at University of Missouri-Kansas City (UMKC), USA, in 2022. He has worked in wireless communication lab as well as multimedia and communication lab in the past. His research interests include immersive video, point cloud and mesh compression, XR, and deep learning solutions for 3D data compression.\end{IEEEbiography}

==> authors_bio_portrait/Geert_Van_der_Auwera_bio.tex <==
\begin{IEEEbiographynophoto}
{Geert~Van~der~Auwera} received the Ph.D. degree in Electrical Engineering from Arizona State University, Tempe, AZ, USA, in 2007, and the Belgian MSEE degree from Vrije Universiteit Brussel (VUB), Brussels, Belgium, in 1997.
Presently, he is a Director at Qualcomm Technologies Inc. in San Diego, CA, USA, in the Multimedia R\&D \& Standards group where he actively contributes to the standardization efforts on MPEG's Dynamic Mesh Compression, Point Cloud Compression and previously on JVET's Versatile Video Coding (VVC). Until Jan. 2011, he was with Samsung Electronics in Irvine, CA, USA. Until Dec. 2004, he was Scientific Advisor with IWT-Flanders, the Institute for the Promotion of Innovation by Science and Technology in Flanders, Belgium. In 2000, he joined IWT-Flanders after researching wavelet video coding at IMEC’s Electronics and Information Processing Department (VUB-ETRO) in Brussels, Belgium. In 1998, his MSEE thesis on motion estimation in the wavelet domain received the Barco and IBM prizes by the Fund for Scientific Research of Flanders, Belgium. His research interests are point cloud compression, XR, video coding, video traffic and quality characterization, video streaming mechanisms and protocols.
\end{IEEEbiographynophoto}

==> authors_bio_portrait/Zhu_Li_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors_bio_portrait/zhu_li_portrait}}]{Zhu Li} is a professor with the Dept of Computer Science \& Electrical Engineering, University of Missouri, Kansas City, and the director of NSF I/UCRC Center for Big Learning (CBL) at UMKC. He received his PhD in Electrical \& Computer Engineering from Northwestern University in 2004. He was AFRL summer faculty at the UAV Research Center, US Air Force Academy (USAFA), 2016-18, 2020-23. He was senior staff researcher with the Samsung Research America's Multimedia Standards Research Lab in Richardson, TX, 2012-2015, senior staff researcher with FutureWei Technology's Media Lab in Bridgewater, NJ, 2010~2012, assistant professor with the Dept of Computing, the Hong Kong Polytechnic University from 2008 to 2010, and a principal staff research engineer with the Multimedia Research Lab (MRL), Motorola Labs, from 2000 to 2008. His research interests include point cloud and light field compression, graph signal processing and deep learning in the next gen visual compression, image processing and understanding. He has 50+ issued or pending patents, 190+ publications in book chapters, journals, and conferences in these areas. He is an IEEE senior member, associate Editor-in-Chief for IEEE Trans. on Circuits \& System for Video Tech, associated editor for IEEE Trans. on Image Processing(2020~), IEEE Trans. on Multimedia (2015-18), IEEE Trans. on Circuits \& System for Video Technology(2016-19). He received the Best Paper Award at IEEE Int'l Conf on Multimedia \& Expo (ICME), Toronto, 2006, and IEEE Int'l Conf on Image Processing (ICIP), San Antonio, 2007.
\end{IEEEbiography}
